LtFi: Cross-technology Communication for RRM between LTE-U and IEEE 802.11

Cross-technology communication (CTC) was proposed in recent literature as a way to exploit the opportunities of collaboration between heterogeneous wireless technologies. This paper presents LtFi, a system which enables to set-up a CTC between nodes of co-located LTE-U and WiFi networks. LtFi follows a two-step approach: using the air-interface LTE-U BSs are broadcasting connection and identification data to adjacent WiFi nodes, which is used to create a bi-directional control channel over the wired Internet. This way LtFi enables the development of advanced cross-technology interference and radio resource management schemes between heterogeneous WiFi and LTE-U networks. LtFi is of low complexity and fully compliant with LTE-U technology and works on WiFi side with COTS hardware. It was prototypically implemented and evaluated. Experimental results reveal that LtFi is able to reliably decoded the data transmitted over the LtFi air-interface in a crowded wireless environment at even very low LTE-U receive power levels of -92dBm. Moreover, results from system-level simulations show that LtFi is able to accurately estimate the set of interfering LTE-U BSs in a typical LTE-U multi-cell environment.

==> packages/config.tex <==
%!TEX root = ../techreport.tex

%\usepackage{fancyhdr}
%\usepackage[centerlast,tight,small]{subfigure}
% the width of a normal figure:
%\newcommand{\figwidth}{\columnwidth*3/4}
\newcommand{\scalefactor}{0.75}

\usepackage{url}
\usepackage{hyperref}
\usepackage{wrapfig}
\usepackage{units}
\usepackage{etoolbox}

\usepackage[printonlyused]{acronym}

% math and calc package
\usepackage{calc}
\usepackage{graphicx}
\usepackage[lined,boxed, vlined,ruled,linesnumbered]{algorithm2e}
\usepackage{amsmath,amssymb,amsthm,amsfonts,amsbsy}

% Document specific packages
%\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{color}
\usepackage[table]{xcolor} % DVI only
\usepackage[caption=false]{subfig}
\usepackage{stfloats}
\usepackage{nicefrac}
%\usepackage{tcolorbox}

\usepackage{multirow}
\usepackage[procnames]{listings}

\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}

\usepackage{soul}
% \usepackage{caption} 
\captionsetup[table]{skip=12pt}

\usepackage{booktabs}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}

\definecolor{BgGray}{gray}{0.7}%
\definecolor{BgGray2}{gray}{0.96}%
\definecolor{RowColorOdd}{named}{BgGray2}%
\definecolor{RowColorEven}{named}{white}%
\definecolor{comments}{gray}{.5}
\definecolor{Gray}{gray}{0.85}
\definecolor{red}{RGB}{160,0,0}
\definecolor{green}{RGB}{0,150,0}
\definecolor{deepblue}{rgb}{0,0,0.5}
\definecolor{deepred}{rgb}{0.6,0,0}
\definecolor{deepgreen}{rgb}{0,0.5,0}


% indent on algorithmic
\newcommand{\IND}[1][1]{\hspace{#1\algorithmicindent}}
\newcommand\colheadbegin{\hline\rowcolor{BgGray}}
\newcommand\colheadend{\\\hline}
\providecommand{\keywords}[1]{\textbf{\textit{Index terms---}} #1}

\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

% FIXME package setup
\usepackage[multiuser,nomargin,marginclue,inline]{fixme}
% use different colors for fixme levels
\fxusetheme{color}
\fxsetup{targetlayout=colorcb}


\widowpenalty=10000
%\clubpenalty=10000

\newcommand\YAMLcolonstyle{\color{red}\mdseries}
\newcommand\YAMLkeystyle{\color{black}\bfseries}
\newcommand\YAMLvaluestyle{\color{blue}\mdseries}

\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{tabularx}
\usepackage{multicol}
\usepackage{graphicx}

\usepackage{tikz}
\usepackage{lipsum}

\usepackage[headsepline,plainheadsepline,footsepline,plainfootsepline]{scrpage2}


\usepackage{mathptmx}
\usepackage[scaled=.92]{helvet}
\usepackage{courier}


% ================================================================
% FIXME package setup
% ================================================================
\usepackage[multiuser,nomargin,marginclue,inline]{fixme}
% use different colors for fixme levels
\fxusetheme{color}
\fxsetup{targetlayout=colorcb}
% define authors for fixme
% \FXRegisterAuthor{commnad prefix}{environment prefix}{tag}
\FXRegisterAuthor{all}{anall}{ALL}
\FXRegisterAuthor{md}{anmd}{MD}
\FXRegisterAuthor{tolja}{antolja}{Tolja}
\FXRegisterAuthor{mc}{anmc}{Mikolaj}
\FXRegisterAuthor{cp}{ancp}{CP}
\FXRegisterAuthor{awo}{anawo}{AWO}
\FXRegisterAuthor{pg}{anpg}{Piotr}

% Usage example \mcfatal{Has to be fixed ASAP}
% Usage example \mcerror{Problem}
% Usage example \mcwarning{Possible problem}
% Usage example \mcnote{Comment}
% fixme mode
% change 'draft' to 'final' for final version
\fxsetup{status=draft}

% and a command for me ;-)
\newcommand\allf{\allfatal}
\newcommand\mdf{\mdfatal}
\newcommand\toljaf{\toljafatal}
\newcommand\mcf{\mcfatal}
\newcommand\cpf{\cpfatal}
\newcommand\awof{\awofatal}
\newcommand\piotr{\pgfatal}
% fixme is dead
\newcommand\copynpaste{\textcolor{BgGray}}
\newcommand\cp{\textcolor{BgGray}}
\newcommand\md{\textcolor{red}}
\newcommand\tolja{\textcolor{red}}
\newcommand\sven{\textcolor{blue}}


% ================================================================
% Page Style
% ================================================================

\usepackage{geometry}
\geometry{a4paper, inner=30mm, outer=25mm, top=40mm, bottom=42mm}


\clearscrheadfoot

\ihead[\Large {\scshape TU Berlin }]{\Large {\scshape TU Berlin }}

\ifoot[{\tiny \begin{minipage}{4.0cm}Copyright at Technische Universität Berlin.\newline All Rights reserved.\end{minipage}}]{{\tiny \begin{minipage}{4.0cm}Copyright at Technische Universität Berlin.\newline All Rights reserved.\end{minipage}}}
\cfoot[\scriptsize \trnumber]{\scriptsize \trnumber}
\ofoot[Page \pagemark]{Page \pagemark}

\pagestyle{scrheadings}

\addtokomafont{pagefoot}{\normalfont}



%\bibliographystyle{plain}


==> packages/tr_cover.tex <==
%!TEX root = ../techreport.tex

% ================================================================
% Cover Sheet
% ================================================================
{
\sffamily

\thispagestyle{empty}

\setlength{\tabcolsep}{0pt} % remove indent within cell
\noindent % remove indent before cell
\begin{tabularx}{\columnwidth}{cXc}
  \includegraphics[height=1cm]{packages/TU-Logo-3D-rot.pdf}
  & &
  \includegraphics[height=1cm]{packages/tknlogo.pdf}
  \\
\end{tabularx}
\setlength{\tabcolsep}{6pt} % back to default

\vspace{1.0cm}

\begin{center}
{\huge
\noindent
Technische Universität Berlin

\vspace{0.5cm}

\noindent
Telecommunication Networks Group

\begin{center}
\rule{15.5cm}{0.4pt}
\end{center}
}
\end{center}

\begin{minipage}[][11.0cm][c]{14.5cm}
{\Huge

\begin{center}
\trtitle
\end{center}

\begin{center}
{\LARGE \trauthor} \\
{\Large \tremail}
\end{center}


\begin{center}
Berlin, \trdate
\end{center}


\vspace{0.5cm}

}


\begin{center}
\setlength{\fboxrule}{2pt}\setlength{\fboxsep}{2mm}
\fbox{TKN Technical Report \trnumber}
\end{center}

\end{minipage}

\setlength{\fboxrule}{0.4pt}
\setlength{\fboxsep}{0.4pt}

\begin{center}

  \rule{15.5cm}{0.4pt}

  \vspace{0.5cm}

  {\huge {TKN Technical Reports Series}}

  \vspace{0.5cm}

  {\huge Editor: Prof. Dr.-Ing. Adam Wolisz}

  \vspace{0.5cm}

 \end{center}


}

